Planar Heyting Algebras for Children 2: Local Operators, J-Operators, and Slashings

Choose a topos $E$. There are several different "notions of sheafness" on $E$. How do we visualize them? Let's refer to the classifier object of $E$ as $\Omega$, and to its Heyting Algebra of truth-values, $Sub(1_E)$, as $H$; we will sometimes call $H$ the "logic" of the topos. There is a well-known way of representing notions of sheafness as morphisms $j:\Omega\to \Omega$, but these `$j$'s yield big diagrams when we draw them explicitly; here we will see a way to represent these `$j$'s as maps $J:H\to H$ in a way that is much more manageable. In the previous paper of this series we showed how certain toy models of Heyting Algebras, called "ZHAs", can be used to develop visual intuition for how Heyting Algebras and Intuitionistic Propositional Logic work; here we will extend that to sheaves. The full idea is this: notions of sheafness correspond to local operators and vice-versa; local operators correspond to J-operators and vice-versa; if our Heyting Algebra $H$ is a ZHA then J-operators correspond to slashings on $H$, and vice-versa; slashings on $H$ correspond to "sets of question marks" and vice-versa, and each set of question marks induces a notion of erasing and reconstructing, which induces a sheaf. Also, every ZHA $H$ corresponds to an (acyclic) 2-column graph, and vice-versa, and for any two-column graph $(P,A)$ the logic of the topos $\mathbf{Set}^{(P,A)}$ is exactly the ZHA $H$ associated to $(P,A)$.

==> edrx15defs.tex <==

% Miscellaneous defs, mostly symbols.
% Edrx, 2005jun25
% Last update: 2010apr20

% (find-doutfile "")
% (find-doutfile "defs-dnt.tex")
% (find-doutfile "defs-headfoot.tex")
% (find-doutfile "defs-sect.tex")
% (find-doutfile "defs-symbols.tex")
% (find-doutfile "defs.tex")


% «.hyp-rules»	(to "hyp-rules")


%
% (find-lsrcfile "base/fontdef.dtx" "rightarrow")

\def\Set{\mathbf{Set}}
\def\Sets{\mathbf{Sets}}
\def\E{\mathbf{E}}
\def\T{\mathbf{T}}
\def\N{\mathbb{N}}
\def\R{\mathbb{R}}
\def\Z{\mathbb{Z}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbH{\mathbb{H}}
\def\bbV{\mathbb{V}}


\renewcommand\O{\mathbf{O}}
\renewcommand\o{\mathbf{o}}
\renewcommand\t{\tau}
\def\typ{\mathbf{t}}
%

% Quantificadores,
%
\def\Exob#1{\mathop{\exists\;{#1}}}
\def\Exbangob#1{\mathop{\exists!\;{#1}}}
\def\Faob#1{\mathop{\forall\;{#1}}}
\def\Ex{\exists}
\def\Exbang{\exists!}
\def\Fa{\forall}

\def\virg{{,\,\,}}
%

% NSA e SSA,
%
%\def\ii{\iota}
\def\ii{\mathbblow{i}}
\def\I{\mathbb{I}}
\def\F{\mathcal{F}}
\def\cofiN{\mathcal{N}}
\def\U{\mathcal{U}}
\def\OO{\mathcal{O}}
\def\jj{\mathbblow{j}}

\def\littlo{o}
\def\bigO{O}


\def\void{\varnothing}
\def\id{\mathrm{id}}
\def\ev{\mathrm{ev}}
\def\cur{\mathrm{cur}}
\def\dom{\mathrm{dom}}
\def\cod{\mathrm{cod}}
%
\def\bsl{\backslash}
\def\phi{\varphi}
\def\False{\Finv}

%%%%
%
% «greek.letters»  (to ".greek.letters")
%
%%%%

\def\aa{\alpha}
\def\bb{\beta}
\def\cc{\gamma}
\def\dd{\delta}
\def\ee{\epsilon}
\def\gg{\gamma}
\def\kk{\kappa}
\def\ww{\omega}
\def\Om{\Omega}
\def\Th{\Theta}
\def\GG{\Gamma}
\def\DD{\Delta}
\def\LL{\Lambda}



% Set_A,
%
\def\A{\mathcal{A}}
\def\SetA{{\bf Set_{\mathcal A}}}

\def\Aplus{{\A^\ast}}
\def\LA{\Lambda_\A}



\def\lbe{{\lambda\beta\eta}}
%\def\lbeto{\underset{\lbe}{\epito}}
\def\lbeto{\epito}
\def\lbeot{{\twoheadleftarrow}}


\def\lbes{{\lambda\beta\eta^\ast}}
%\def\lbeto{{\epito^\ast}}



\def\SetI{{\Set^{\mathbb{I}}}}
\def\SetF{{\Set^{\mathcal{F}}}}
\def\SetU{{\Set^{\mathcal{U}}}}
\def\SetP{{\Set^{\mathbf{P}}}}
\def\SetM{{\Set^{\mathbf{M}}}}
\def\SetC{{\Set^{\bf C}}}
\def\Top{{\bf Top}}
\def\PTop{{\bf PTop}}
\def\Vect{{\bf Vect}}
\def\Grp{{\bf Grp}}
\def\Mon{{\bf Mon}}
\def\catA{\mathbf{A}}
\def\catB{\mathbf{B}}
\def\catC{\mathbf{C}}
\def\catD{\mathbf{D}}
\def\catE{\mathbf{E}}
\def\catH{\mathbf{H}}
\def\catI{\mathbf{I}}
\def\catJ{\mathbf{J}}
\def\catP{\mathbf{P}}
\def\OX{{\mathcal{O}_X}}

\def\calA{\mathcal{A}}
\def\calB{\mathcal{B}}
\def\calC{\mathcal{C}}
\def\calD{\mathcal{D}}
\def\calE{\mathcal{E}}
\def\calF{\mathcal{F}}
\def\calG{\mathcal{G}}
\def\calL{\mathcal{L}}
\def\calN{\mathcal{N}}
\def\calR{\mathcal{R}}
\def\calV{\mathcal{V}}

% Coisas para o capítulo sobre análise não-standard
%
% (find-lsrcfile "amsmath/amsmath.dtx" "\\newcommand{\\sideset}[3]")

\makeatletter
\def\sidesetscript#1#2#3{%
  \@mathmeasure\z@\scriptstyle{#3}%
  \global\setbox\@ne\vbox to\ht\z@{}\dp\@ne\dp\z@
  \setbox\tw@\box\@ne
  \@mathmeasure4\scriptstyle{\copy\tw@#1}%
  \@mathmeasure6\scriptstyle{#3\nolimits#2}%
  \dimen@-\wd6 \advance\dimen@\wd4 \advance\dimen@\wd\z@
  \hbox to\dimen@{}\mathop{\kern-\dimen@\box4\box6}%
}
\makeatother
%
\def\B{\mathcal{B}}
\def\interfin{\bigcap_{\rm fin}}
\def\ns#1{\sideset{^*}{}{\mathop{#1}}}
\def\nss#1{\sidesetscript{^*}{}{\mathop{#1}}}
\def\raiseset{\mathord{\uparrow}}
\def\Pts{\mathcal{P}}


% Combinadores,
%
\def\cbS{\mathbf{S}}
\def\cbK{\mathbf{K}}
\def\cbI{\mathbf{I}}
\def\cbP{\mathbf{P}}
\def\cbD{\mathbf{D}}
\def\cbV{\mathbf{V}}
\def\cbT{\mathbf{T}}
\def\cbF{\mathbf{F}}
\def\SKI{\mathbf{SKI}}
\def\app{\operatorname{app}}


% Conectivos,
%
% (find-fline "/usr/lib/texmf/tex/latex/misc/program.sty" "poor man's bold")
% (find-fline "/usr/lib/texmf/tex/latex/amslatex/amsbsy.sty" "pmb")
% (find-fline "/usr/lib/texmf/tex/latex/amslatex/amstex.sty" "pmb")
% (find-fline "/usr/lib/texmf/tex/latex/tools/bm.sty" "pmb")
%\def\pmb{\protect\ppmb}
%\def\ppmb#1{\setbox0=\hbox{\bf #1}
%            \kern-.025em\copy0\kern-\wd0
%           \kern.05em\copy0\kern-\wd0
%           \kern-.025em\raise.0433em\box0 }}
\def\LAND{\pmb{\land}}
\def\LOR{\pmb{\lor}}
\def\TO{\pmb{\to}}
\def\TO{\funto}



\let\sweddot\r

% Tipos,
%
\def\nn{\mathbblow{n}}
\def\r{\mathbblow{r}}
\def\z{\mathbblow{z}}
\def\lefto{\mathcal{L}}
\def\righto{\mathcal{R}}

\def\compr{\operatorname{compr}}
\def\Int{\operatorname{Int}}

\def\mon{{\mathop{[\;]}}}

\def\setof#1{\{\,#1\,\}}
%\def\setofst#1#2{\,\setof{{#1}\;|\;{#2}}\,}
\def\setofst#1#2{\{\,#1\;|\;#2\,\}}

\def\adj{\operatorname{adj}}

\def\conetr#1#2#3{(\O_{#3},\, #3 \to #1,\, #3 \to #2)}
\def\coneab#1{\conetr{a}{b}{#1}}

\def\ang#1{\langle #1 \rangle}
\def\angc{\ang{\,,}}
\def\llangle{\langle\!\langle}
\def\rrangle{\rangle\!\rangle}
\def\angg#1{\llangle#1\rrangle}



\def\hom{\operatorname{hom}}
\def\Hom{\operatorname{Hom}}
\def\op{{\operatorname{op}}}
\def\und#1{{\underline{#1}}}
\def\Cat{\mathbf{Cat}}
\def\colim{{\operatorname{colim}}}
\def\Colim{{\operatorname{Colim}}}
\def\Lim{{\operatorname{Lim}}}

\def\welldef{{\operatorname{wd}}}
\def\welld{{\operatorname{wd}}}

\def\ssapp#1#2{(#1,#2)\text{-app}}
\def\ssabs#1#2{(#1,#2)\text{-abs}}

\def\Props{\operatorname{Props}}
\def\Prfs {\operatorname{Prfs}}
\def\prf  {\operatorname{prf}}
\def\Objs {\operatorname{Objs}}

\def\comp {\operatorname{comp}}
\def\src  {\operatorname{src}}
\def\tgt  {\operatorname{tgt}}
\def\fv   {\operatorname{fv}}
\def\FV   {\operatorname{FV}}
\def\dom  {\operatorname{dom}}
\def\Cod  {\operatorname{Cod}}
\def\Sub  {\operatorname{Sub}}
\def\CanSub{\operatorname{CanSub}}





% Bananas
\def\ban#1{(\mskip-1.2\thinmuskip| #1 |\mskip-1.2\thinmuskip)}

\def\<{\langle}
\def\>{\rangle}



% «hyp-rules»  (to ".hyp-rules")
% Rules for hyperdoctrines (2010apr18)
%
\def\nat     {\natural}

\def\sen   {\operatorname{sen}}
\def\arcsen{\operatorname{arcsen}}
\def\sec   {\operatorname{sec}}
\def\arcsec{\operatorname{arcsec}}

% \def\cur  {\operatorname{cur}}
% \def\uncur{\operatorname{uncur}}
\def\cur  {\operatorname{\textsf{cur}}}
\def\uncur{\operatorname{\textsf{uncur}}}







% Local Variables:
% coding:               raw-text-unix
% ee-delimiter-percent: "\n%\n"
% ee-anchor-format:     "«%s»"
% End:


==> edrxheadfoot.tex <==
% This is the file "examples/edrxheadfoot.tex" of dednat4.
% See: http://angg.twu.net/dednat4.html
%      http://angg.twu.net/dednat4/examples/edrxheadfoot.tex
%      http://angg.twu.net/dednat4/examples/edrxheadfoot.tex.html
% Author: Eduardo Ochs <eduardoochs@gmail.com>
% Version: 2008oct09
% Public domain.
%
% This doesn't have much to do with dednat4, but let me explain. :-)
% I "\input" this file from most of my LaTeX files. It changes the
% code for headers and footers to make the page number appear in the
% header and the filename (the "\jobname", actually) and the date of
% the compilation appear of at the footer. Including it in dednat4
% made some examples easier to write.
%   (find-dn4ex "edrxmain41.tex")
%   (find-dn4ex "edrxmain41a.tex")

% (find-lsrcfile "base/ltpage.dtx"      "Page Style Commands")
% (find-source2epage (+ 9 360) "65.1     Page Style Commands")
% (find-source2etext           "65.1     Page Style Commands")
% (find-lshortfile "src/things.tex"  "Page Styles")
% (find-lshorttext           "1.6.3   Page Styles")
% (find-lshortpage (+ 14 13) "1.6.3   Page Styles")
% (find-es "tex"      "book.cls")
% (find-lsrcfile "base/book.cls"   "\\if@twoside" "\\def\\ps@headings")
% (find-source2efile "classes.dtx" "\\if@twoside" "\\def\\ps@headings")
% (find-source2efile "classes.dtx" "The page style")
% (find-source2efile "classes.dtx" "<!book>\\pagestyle{plain}")
% (find-source2efile "nfssfont.dtx" "time")
%
\makeatletter
\newcount\m \newcount\n
\def\twodigits#1{\ifnum #1<10 0\fi \number#1}
\def\hours{\n=\time \divide\n 60
  \m=-\n \multiply\m 60 \advance\m \time
  \twodigits\n:\twodigits\m}
%
\def\draftfooter{\jobname{} \today{} \hours}
\def\footertext{\draftfooter}
\def\ps@headings{%
  \def\@oddfoot{\hfil \footertext \hfil}
  \let\@evenfoot\@oddfoot
  \def\@oddhead{{\slshape\rightmark}\hfil\thepage}%
  \let\@mkboth\markboth
  \def\chaptermark##1{%
    \markright {\MakeUppercase{%
      \ifnum \c@secnumdepth >\m@ne
        \if@mainmatter
          \@chapapp\ \thechapter. \ %
        \fi
      \fi
      ##1}}}}
\ps@headings
\makeatother
%
\def\shorttoday{%
  \number\year%
  \ifcase\month\or jan\or feb\or mar\or apr\or may\or
     jun\or jul\or aug\or sep\or oct\or nov\or dec\fi
  \twodigits\day}
\def\edrxnotesfooter#1{{\tiny #1 (typeset \shorttoday{} \hours)
  {\tt Edrx http://angg.twu.net/}}}
\def\edrxnotes#1{\gdef\footertext{\edrxnotesfooter{#1}}}
\def\noedrxfooter{\gdef\footertext{}}
%
% (find-es "tex" "edrxnotes")
% (find-fline "/usr/share/texmf-tetex/tex/generic/babel/portuges.ldf")
% (find-fline "/usr/share/texmf-tetex/tex/generic/babel/portuges.sty")






% Local Variables:
% coding:               raw-text-unix
% ee-delimiter-percent: "\n%\n"
% ee-anchor-format:     "«%s»"
% End:

